Evaluating List Construction and Temporal Understanding capabilities of Large Language Models

Large Language Models (LLMs) have demonstrated immense advances in a wide range of natural language tasks. However, these models are susceptible to hallucinations and errors on particularly temporal understanding tasks involving multiple entities in answers. In such tasks, they fail to associate entities with accurate time intervals, generate a complete list of entities in answers or reason about events associated with specific temporal bounds. Existing works do not extensively evaluate the abilities of the model to perform implicit and explicit temporal understanding in a list answer construction setup. To bridge this gap, we propose the Time referenced List based Question Answering or TLQA benchmark that requires structured answers in list format aligned with corresponding time periods. Our TLQA benchmark, requires both list construction and temporal understanding simultaneously, which to the best of our knowledge has not been explored in prior benchmarks. We investigate the temporal understanding and list construction capabilities of state-of-the-art generative models on TLQA in closed-book and open-domain settings. Our findings reveal significant shortcomings in current models, particularly their inability to provide complete answers and temporally align facts in a closed-book setup and the need to improve retrieval in open-domain setup, providing clear future directions for research on TLQA. The benchmark and code at https://github.com/elixir-research-group/TLQA.

==> fig/intro-fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/scatter-plot.pdf}
    \vspace{-3em}
    \caption{The distribution of retrieval and ranking scores of the retrieved documents. the green region represents the documents selected in the telescoping for ranking. The green documents are selected on the basis of online relevance estimation. The ground truth documents are explicitly labelled as ``relevant''.}
    \label{fig:intro-1}
    \vspace{-1em}
\end{figure}

==> fig/schematic-algo.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/cerebrus-algo-schematic.pdf}
    \caption{Schematic figure of the Online relevance estimation algorithm.}
    \vspace{-3.5em}
    \label{fig:ORE}
\end{figure}

==> framework.tex <==


\section{Online Relevance Estimation}
\label{sec:method}


In this section, we describe our framework for online relevance estimation (\cerberus{}). We depart from standard telescoping approaches where document candidate space is pruned using less precise retrievers to select documents for further ranking. However, these approaches suffer from the \textit{bounded recall} problem. Hence, approaches that rely on the first-stage retrieval results ignore relevant documents that may have been missed in these stages due to low retrieval scores. 
% Recent works~\cite{macavaney2022adaptive, kulkarni2023lexically, Kulkarni2024lexboost, rathee2024quam} have proposed adaptive retrieval to overcome the \textit{bounded recall problem} but heuristics mechanism of prioritizing the candidate documents is biased towards the first-stage retrieved documents.
However, it is essential to carefully prioritize documents from the large document space by determining their potential value for the expensive ranking stage, owing to the limited budget of the final result list.

% The existing approaches for adaptive retrieval primarily rely on heuristics to select documents to rank, such as alternating between the initial retrieved list and the neighborhood. 

\cerberus{} is a selective exploration-based approach designed according to this philosophy to schedule the most important documents for ranking from the entire candidate documents space. We drew inspiration from pure exploration-based approaches for Multi-Arm Bandits (MAB) \cite{LUCB,ucb}. We estimate the utility of each candidate document (arm) by leveraging features broadly categorized as query-document affinity (\textsc{Q2DAff}), document-document affinity (\textsc{D2DAff}), and affinity of candidate document to highly relevant re-ranked documents. This utility is termed \textit{estimated relevance} which is iteratively updated using an online approach. This serves as an approximation to actual relevance scores from an expensive ranker.




\input{cerberus_algorithm}

\input{tables/features}


\subsection{The ORE framework}
\label{sec:framework}

In this section, we present the general algorithmic framework for online relevance estimation. 
We further expand upon the details of specific features employed and related details for hybrid and adaptive retrieval setups in Section \ref{sec:estimated rel}.
Since, the retrieval set is large, it is infeasible to rank all documents using an expensive scorer. 
While traditional telescoping approaches employ retrieval scores for filtering documents, this has limitation as stated earlier. Hence, it is crucial for determining the utility of the candidate documents online while minimizing calls to expensive ranker.



Our goal is to perform a careful selection of potentially relevant documents while being sample efficient. This problem is analogous to the top-$l$ arms selection problem in stochastic linear bandits \cite{LUCB,chaudhuri2019pac}. 
In the current setting, the arms correspond to the documents, and feature vectors for the linear bandit are a combination of features in Table \ref{tab:features}. The reward in our setting can be thought of as the actual relevance of a candidate document from an expensive ranker. Our main objective is to prioritize the documents to be included in the final rank list while reducing calls to the expensive ranker.

To this end, we start with the retrieved list from initial stage and construct a pool of candidate documents, depending on the retrieval setup (hybrid or adaptive). Next, we use the features (defined in Table~\ref{tab:features}) to estimate the relevance of each candidate document. For given query $q$ and a candidate document $d$, let $\phi(q,d)$ be the ranker's relevance score (or actual relevance) which is analogous to rewards in linear stochastic bandits setting. Let $\textsc{EstRel}(\vec{\alpha},\vec{x})$ be the estimated relevance score using \cerberus{} which aims to approximate the actual relevance from the expensive ranker. The $\vec{x}$ is the feature vector and $\vec{\alpha}$ is vector of learnable parameters. The \textsc{EstRel} scores are similar to rewards for arms 
% During re-ranking, we learn the parameters, $\vec{\alpha}$, by minimizing the uncertainty error between the ranker's relevance and estimated relevance:

\begin{equation}
    \textsc{EstRel}(\vec{\alpha},\vec{x}_d) = \vec{\alpha}\cdot \vec{x}_{d}^{T}
    \label{eq:EstRel}
\end{equation}
Our document selection of prioritization task primarily involves learning the parameters $\alpha$'s of the relevance estimation function. This entails carefully selecting the documents to be scored by the expensive ranker and computing the approximation error between estimated relevance scores and actual relevance scores from the ranker as follows:
\begin{equation}  
E(\vec{\alpha}; q, d, \vec{x}_d) = \frac{1}{2} \| \phi(q, d) - \textsc{EstRel}(\vec{\alpha}, \vec{x}_d) \|^2
\label{eq:error}
\end{equation}

Usually in linear stochastic bandits, the proposed approaches for top-$l$ arm selection pull an arm in each round to update the learnable parameters of the reward estimator \cite{LUCB}. This subsequently leads to revised reward estimates for all arms. However, the classical setting in MAB is not directly suitable for our setting as they  require at least linear time in the number of arms, in each round till convergence.


Hence, we depart from the classical linear stochastic bandit approaches by constraining the calls to expensive ranker (arm pulls) on a budget for number of samples to be scored ($m$). 
During re-ranking using the expensive ranker, we update the parameters $\vec{\alpha}$ only for the given budget of $m$ (a hyperparameter) batches. For the remaining batches, we use the learned parameters to get the estimated relevance for each document in the batch and add them to final ranked list based on the estimated relevance. The intuition behind employing estimated relevance for ranking the rest of the documents is that the estimated scores would serve as a proxy for actual relevance scores through our iterative parameter updates.

This results in a more sample efficient online relevance estimator which uses less calls to the ranker during parameter estimation stage and the ranking stage.


% \subsection{Online Query Processing using \cerberus{}}

\subsection{
Query Processing using \cerberus{}}

Algorithm~\ref{algo:cerberus} provides an overview of how adaptive retrieval for a query is performed through the proposed \cerberus{} method.  Let $q$ be the given query and let $R_0$ be the initial pool of retrieved results, and $R_1$ be the final re-ranked pool of documents (initially empty). Let $S$ be the set of top $s$ documents that we have re-ranked so far. Let $b$ be the batch size and $c$ be the re-ranking budget. Let $A$ be the pool of documents (arms) that can be initialized with initial retrieved results (Hybrid vs. adaptive retrieval). Let $\vec{x}_d$ be the features vector of document $d$ in $A$. Each document (arm) in $A$ is assigned with \textit{estimated relevance score}, \textsc{EstRel}, (using Equation~\ref{eq:EstRel}) with $\vec{\alpha}_{1}$ which is initialized randomly from a normal distribution ($\vec{\alpha}_{1} \gets N(0,1)$). The \textsc{EstRel} score indicates the utility or perceived importance of each candidate document (arm) in $A$.

Given a query $q$, \cerberus{} initially starts with taking a batch $B$ of top $b$ documents from the pool of documents (arms) $A$. These documents are scored using scorer (e.g., MonoT5~\cite{nogueira2020document}) and added to $R_1$. Then subsequently, \cerberus{} adds new documents (arms) into the candidate pool $A$ by exploring the neighborhood graph (in adaptive) or exploring the retrieval depth (in Hybrid).  

To determine the documents that need to be prioritized for scheduling, we first compute \textit{estimated relevance} \textsc{EstRel} using Equation \ref{eq:EstRel}. This is followed by the selection of top $b$ documents (arms) from $A$ based on their \textsc{EstRel} scores. This is followed by the ranking stage, where the batch $B$ is scored using the expensive ranker (e.g., MonoT5). Next, the parameters, $\vec{\alpha}$, are updated using the uncertainty error defined in Equation~\ref{eq:error}. Further, the \textsc{EstRel} scores are updated using the updated parameters, $\vec{\alpha}$. The expensive ranker is used only until the condition  $|R_1|<m* b$ is met. For the remaining documents, the learnt parameters, $\vec{\alpha}$, are re-used and the batch of documents is selected using the \textsc{EstRel} scores. Next, the documents from the selected batch are added to the final rank list $R_1$. We keep updating the \textsc{EstRel} scores of candidate documents and selecting the batch until the $|R_1|<c$ condition is met.
The intuition behind scoring only a part of the documents is that the actual relevance for a candidate document can be approximated using a learned combination of its features. Hence, by scoring some of the initial batches of documents prioritized for scoring, we can obtain good relevance estimates using our formulation detailed in Section \ref{sec:estimated rel} for other candidate documents. This obviates the need for expensive scorer calls until the budget is fulfilled, providing efficiency gains without significantly impacting performance, as shown in our experimental results.


% \subsection{Online Query Processing using \cerberus{}}

% Algorithm~\ref{algo:cerberus} provides an overview of how adaptive retrieval for a query is performed through the proposed \cerberus{} method.  Let $q$ be the given query and let $R_0$ be the initial pool of retrieved results, and $R_1$ be the final re-ranked pool of documents (initially empty). Let $S$ be the set of top $s$ documents that we have re-ranked so far. Let $b$ be the batch size, $c$ be the re-ranking budget and $G_a$ be the learnt affinity graph (of \laff{} graph). Let $A$ be the pool of documents (arms) initialized with $R_0$. 

% Given a query $q$, \cerberus{} initially starts with taking a batch $B$ of top $b$ documents from the pool of documents (arms) $A$. These documents are scored using scorer (e.g., MonoT5~\cite{nogueira2020document}) and added to $R_1$. Then subsequently, the neighbors of this first batch $B$ are looked up from the \laff{} graph $G_a$ and added to the pool of documents (arms) $A$ to expand the pool of candidate documents (arms) to be selected for adaptive retrieval.

% To determine the documents that need to be prioritized for adaptive retrieval, we first select the top $s$ documents from the pool of re-ranked documents so far $R_1$. This is followed by computation of \textit{estimated relevance} \textsc{EstRel} using Equation \ref{eq:EstRel}, which indicates the utility or perceived importance of each candidate document (arm) from $A$. This is followed by the selection of top $b$ documents (arms) from $A$ based on their \textsc{EstRel} scores. 

% This is followed by the ranking stage, where all batches $B$ are scored using the expensive ranker. Alternatively, only a portion of batches is scored till the condition $|R_1|<c$ is met with the rest of the batches being assigned their estimated relevance scores ($\textsc{EstRel}$). The intuition behind scoring only a part of the documents is that the \textsc{EstRel} for a candidate document can be partly approximated using the average relevance of documents in its neighborhood that have already been scored. Hence by scoring some of the initial batches of documents prioritized for scoring, we can obtain good relevance estimates using our formulation detailed in Section \ref{sec:estimated rel} for other candidate documents that are in their neighborhood. This obviates the need for expensive scorer calls till the budget for adaptive retrieval is fulfilled, providing efficiency gains without significantly impacting performance, as shown in our experimental results.



==> intro.tex <==
\section{Introduction}
\label{sec:intro}
The standard relevance modelling task of providing information for a given user's query follows a two-stage (also called \textit{cascading}) process. The first stage efficiently retrieves (e.g., using lexical matching) a few documents from the huge corpus. In the second stage, an expensive ranker (e.g., MonoT5) is used to re-rank these documents.


Finally, only a few top documents are shown to the user. But, in this \textit{cascading} pipeline, if a relevant document is missed during the first stage retrieval, it can not be shown to the user after the re-ranking.

In literature, this is termed as \textit{bounded recall problem}.

To solve this bounded recall problem, recent adaptive retrieval based methods are proposed~\cite{macavaney2022adaptive,kulkarni2023lexically, rathee2024quam, Kulkarni2024lexboost, macavaney2024splaid}. 

These approaches make use of document-document similarities which are encoded by a graph (called \textit{corpus graph}). This \textit{corpus graph} is built offline and based on the \textit{Clustering Hyptothesis}~\cite{jardine1971use}, which says documents close to each other tend to answer the same query. 

So, instead of simply re-ranking initial results,  the documents from the neighbors (in the \textit{corpus graph}) of the top re-ranked documents are scheduled in alternating iterations of re-ranking. This alternating paradigm can add relevant documents to the final results. Also, these approaches only add minimal latency costs in comparison to the latency of the expensive ranker.


However, methods like \gar{}~\cite{macavaney2022adaptive} and LADR~\cite{kulkarni2023lexically} do not use the degree of similarities between the documents and do not fully exploit the graph neighborhood, i.e., only the first few documents in the neighbors get the opportunity to be scheduled in the iteration. To overcome the neighborhood selection problem, \quam{}~\cite{rathee2024quam} proposed to use query affinity modelling by using the degree of similarity between documents and all neighbors get equal opportunity to get scheduled. However \quam{} also uses an alternating strategy between initial results and neighborhood. Consequently, the design of the algorithm forces to select documents of initial results, even if they are not relevant to the query. 

Further, existing re-ranking approaches, including standard re-ranking and adaptive re-ranking (or adaptive retrieval) call the expensive ranker for all documents for a given re-ranking budget. 

\input{plots/ar_plots}

To tackle the above-mentioned problems (biasness towards initial retrieved results and the number of calls of expensive ranker), we propose a principled approach called \cerberus{}, a multi arms bandit based adaptive retrieval approach. \cerberus{} explores the initial retrieved results and exploits the neighbors of the top re-ranked documents and creates a growing pool of candidate documents (arms). In the pool of documents (arms), each document gets the opportunity to be scheduled for re-ranking. Our proposed method \cerberus{} learns an online policy to estimate the expensive ranker's score for each candidate document. Our proposed approach is sample efficient, i.e., given the true ranker's scores of enough documents, \cerberus{} can approximate the scores for remaining documents using the online learnt policy. 

\mpara{Key Contributions:}

\begin{itemize}
    \item We propose a principled approach, \cerberus{} .
    
    \item 

    \item 
    We perform experiments to show the effectiveness and efficiency of our method in comparison to standard re-ranking and adaptive re-ranking (adaptive retrieval) baselines. 

\end{itemize}


We release the code of our work at \url{}.

==> method.tex <==

 \vspace{-1em}
\section{Estimated Relevance in \cerberus{}}
\label{sec:estimated rel}

 Relying only on retrieval scores (\textsc{Q2DAff}) would lead to omission of documents which might be relevant, as shown in Figure \ref{fig:intro-1}. However, these documents may have closer proximity to documents already deemed relevant as measured by document-document similarity/affinity (\textsc{D2DAff}). If we compute the affinity of the document with respect to a set of documents, it is termed as \textsc{D2SETAff}. 
 
 Hence, the choice of features used in \cerberus{} is the cornerstone of quality in online relevance estimation. A summary of features employed in \cerberus{} in different setups (hybrid and adaptive) is as shown in Table \ref{tab:features}. Apart from \textsc{Q2DAff} scores, we also capture the proximity of the document to a small set of documents already deemed relevant by the expensive ranker. The intuition follows from the explore-exploit paradigm of linear stochastic bandits. In the current setting, our goal is to allow for the balance between prioritizing documents with high retrieval scores (exploitation) or provisioning selection of documents which have closer proximity to highly relevant documents despite it's lower retrieval scores (exploration). Note that, \cerberus{} is not limited to only the features in the Table \ref{tab:features}. The design of \cerberus{} algorithm makes it flexible towards the addition of new features. 

For a given query $q$, let $R_0$ be the initial retrieved results with lexical ($x_1$) or semantic ($x_2$) query-document similarities, \textsc{Q2DAff}. and $R_1$ be the results after re-ranking. Let $G_c$ be the corpus graph. The corpus graph $G_c$ encodes lexical ($x_4=BM25(d,d^\prime)$) or semantic ($x_5=TCT(d,d^\prime)$) document-document similarities, \textsc{D2DAff}. Let $G_a$ be the learnt affinity graph, proposed in \quam{}~\cite{rathee2024quam}, which encodes learnt affinity, \laff{} scores ($x_6$).

\subsection{Hybrid Retrieval using~\cerberus{}}
Hybrid retrieval usually entails employing multiple lexical (BM25) and dense (TCT) retrievers for a high retrieval depth, followed by rank fusion to merge the retrieved lists. These approaches then usually cap the merged results to a lower retrieval depth, ignoring other potentially relevant documents with lower retrieval scores. However, \cerberus{} promotes exploration by constructing a candidate pool of documents from the entire merged list. In the hybrid retrieval setup, our goal is to prioritize not only documents with high retrieval scores (\textsc{Q2Daff}) but also balance the exploration of documents that are in close proximity to documents (\textsc{D2DAff}) already deemed highly relevant. Hence, we carefully select the features from Table \ref{tab:features} reflective of this philosophy

\[\Call{Q2DAff}{q,d} = \alpha_1 * BM25(q,d) + \alpha_2 * TCT(q,d)\] $\forall d \in \mathcal{D}_q$, where $\alpha_1, \alpha_2 \in \vec{\alpha}$.

For \textsc{D2DAff} features in the hybrid retrieval context, we employ both lexical (RM3 i.e., $x_3$) and semantic scores ($TCT(d,d^\prime)$, i.e., $x_5$). It is critical to note that these \textsc{D2DAff} scores are employed to compute \textsc{D2SetAff} scores, which measure the proximity of a candidate document to a set of highly relevant documents. These highly relevant documents are selected as top-s documents that have already been scored so far from $R_1$.
\[ \textsc{D2SetAff}=\alpha_3 * RM3(q^\prime,d) + \alpha_4 * \frac{\sum_{d^\prime \in S} (\phi(q,d^\prime) *TCT(d,d^\prime))}{|S|}\]
where $\alpha_3, \alpha_4 \in \vec{\alpha}$ and $q^\prime$ is the expanded query by using $RM3$ expansion over top re-ranked documents so far in $R_1$. Note, we simply look up the score of $\phi(q,d^\prime)$ since $d^\prime$ is already re-ranked using ranker $\phi$. Mapping this to Equation~\ref{eq:EstRel}, \textsc{EstRel} is computed using $\vec{\alpha}=[\alpha_1,\alpha_2,\alpha_3,\alpha_4]$ and $\vec{x}_d$=[$x_1$, $x_2$, $x_3$, $x_5$]. The parameters in $\vec{\alpha}$ are learnt using the mechanism described in Section 3.1 and Algorithm \ref{algo:cerberus}. 

%\mpara{Query-Document Affinity.} 
%Given a candidate document $d$, it's affinity to the original query $q$ is defined as the degree of relevance indicated by the scores from first-stage retrieval.  For instance, if BM25 is employed for first-stage retrieval, query-document affinity,  \textsc{Q2DAff}

\subsection{Adaptive Retrieval using \cerberus{}}

We adopt a similar philosophy for document prioritization in the adaptive retrieval setup. However, adaptive retrieval is a bit more involved, as the candidate pool $\mathcal{D}_q$ is not static and expands with the addition of neighbors of top-scored documents. Hence, the relevance estimation for the candidate documents is linear in terms of number of documents (arms). Hence, we draw inspiration from top-$l$ arm selection in linear stochastic bandits like LUCB \cite{LUCB} and GIFA \cite{reda2021top} which maintain multiple sets such as : 1) arms with high reward estimates and 2) arms with low reward estimates to balance exploration. However, these approaches still sample actual rewards for one arm from each of these lists, rendering them computationally infeasible for a large candidate pool.
Hence, we maintain two shortlists which represent 1) documents (arms) with high \textsc{Q2Daff} scores, denoted by $U \subset \mathcal{D}_q$, and 2) documents with high \textsc{D2SetAff} scores, denoted by $V\subset \mathcal{D}_q$. The intuition is that since \textsc{EstRel} primarily depends on balancing between documents with high \textsc{Q2Daff} and documents with high  \textsc{D2SetAff} scores maintaining shortlists based on these measures help reduce the expanding candidate space and also reduce the impact of documents with noisy estimates.


In the adaptive setting, $\Call{Q2DAff}{q,d} = BM25(q,d)$. Given a document affinity graph $G_a$, the document-document affinity is given by: $\Call{D2DAff}{d,d^\prime } = G_a(d,d^\prime) $ where  $G_a(d,d^\prime)$ is the edge weight or edge affinity between the source document $d$ and its neighbor $d^\prime$ in the corresponding graph. Note that, we lookup \textsc{Q2Daff}(q,d) and \textsc{D2DAff}(q,d) and compute \textsc{EstRel} $\forall$ $d \in U \cup V$ thereby providing an efficient relevance estimation mechanism.
Our goal is to primarily balance the exploitation paradigm with the exploration. The exploitation primarily entails selecting documents that have high affinity to the query. Whereas, the exploration paradigm entails scheduling neighbors that may not have high affinity to the query but are closely related to multiple documents deemed to be highly relevant to the query. To accomplish this, we compute the affinity of the candidate document to the ranked set of documents $S$, denoted as \textsc{SetD2DAff} and defined as
\begin{equation}
\Call{D2SetAff}{d, S} =\frac{\sum_{d^\prime \in S \cap N_d} (\textsc{D2DAff}(d, d^\prime))} {|S \cap N_d|}
\label{eq:SetD2Daff}
\end{equation}
where $N_d = \Call{Neighbours}{d, G_a}$ is the set of neighbors of document $d$ in the learnt affinity graph $G_a$. The estimated relevance ($\textsc{EstRel}$) of the candidate document $d$ to the given query $q$ can be better estimated using an average of the relevance (score given by the ranker $\phi$) of documents from $S$ in its neighborhood that are already deemed to be highly relevant to the query. Hence we also include this new feature in adaptive retrieval as it naturally fits into the neighborhood-based retrieval philosophy of this setup. 


% where $P(Rel(d^{\prime}))$ encodes the estimated relevance distribution induced by a relevance scorer (e.g., MonoT5~\cite{nogueira2020document}) model.
% $P(R(d^{\prime}))$ can be estimated in multiple ways. 
% We let $P(Rel(d^{\prime})) =\frac{e^{\phi\left(q,d\right)}}{\sum_{d^{\prime} \in S} e^{\phi\left(q,d^{\prime} \right)}}$.

% \mpara{Utility of the document.} To balance the query-document affinity and document-document set affinity, we interpolate \textsc{Q2DAff} and \textsc{SetD2DAff}.
% The interpolated measure is the estimated utility of a candidate document $d$ defined as
% \begin{equation}
% \Call{U}{q,d,S}= \alpha \cdot \Call{Q2Daff}{q,d}  + \beta \cdot \Call{SetD2DAff}{d, S}
% \label{eq:utility}
% \end{equation}
% where $\beta$, s.t.  $0\leq\beta\leq 1$, is a parameter for interpolation. 



\begin{equation}
x_7 = \frac{\sum_{d^\prime \in S \cap N_d}{\Call{Score}{q,d^\prime}}}{|S \cap N_d |}
\end{equation}

Hence, the features can be combined in the following form for adaptive retrieval: 
\vspace{-0.1cm}
\[\alpha_1 * \textsc{Q2DAff}(q,d) + \alpha_2 * \textsc{D2SetAff}(q,d)  + \alpha_3 * x_7\]
\vspace{-0.5cm}
\begin{equation}
  \Call{Score}{q,d^\prime} =  \begin{cases} 
       \phi{(q, d^\prime )} + \psi(q, d^\prime ) \ ; \ if \ d^\prime \ is \ scored \ using \ \phi \\
        \Call{EstRel}{\vec{\alpha},\vec{x}_d} \ ; \ otherwise \\
   \end{cases}
\label{eq:score}
\end{equation}
where $\psi$ is a dual encoder\footnote{We use inexpensive dual encoder, TAS-B~\cite{hofstatter2021efficiently} for better numerical stability.} and $S^\prime$ is set of top $s$ documents in previous iteration. We look up the scores from $\phi$, since the documents are already in $R_1$ ($d^\prime\in S^\prime \subseteq R_1$). Mapping this to Equation~\ref{eq:EstRel}, \textsc{EstRel} is computed using $\vec{\alpha}=[\alpha_1,\alpha_2,\alpha_3]$ and $\vec{x}_d$=[$x_1$, $x_6$, $x_7$]. %These  parameters in $\vec{\alpha}$ are learned using the mechanism described in Section 3.1 and Algorithm \ref{algo:cerberus}.

% The above measure is termed \textit{estimated relevance}, $\textsc{EstRel}$, and is used as a proxy for the importance of a document. The documents with high $\textsc{EstRel}$ scores are scheduled for ranking. This score balances the notion of affinity to query and affinity to highly relevant documents. It allows for principled exploration of useful documents that may not have a high affinity to query but have high document affinity, $\textsc{D2DAff}$ to the neighbors of re-ranked documents in the set $S$, while balancing exploitation of documents with high affinity to query, $\textsc{Q2DAff}$.


Note that all the above computations for hybrid or adaptive retrieval setups are vectorized and computed for a batch of documents at a time. We present at the document level for ease of understanding. Also, note that $ \mathcal{D}_q$ get updated after scoring each batch $B$ with the neighbors in $G_a$ of each document $d \in B$, i.e., $ \mathcal{D}_q$ $\gets$ $\mathcal{D}_q$  $ \cup$ \Call{Neighbors}{$d$,$G_a$}, but we maintain shortlists as discussed earlier.  

% \subsection{Offline Policy for Multi-Arm-Bandit framework}








==> ndcg_plots.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/ndcg_plot.png}
    \caption{Comparison of retrieval models (nDCG) }
                \label{fig:retriever_extra_2}

\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/recall_plot.png}
    \caption{Comparison of retrieval models (Recall) }
                \label{fig:retriever_extra_1}

\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/precision_plot.png}
    \caption{Comparison of retrieval models (Precision). }
        \label{fig:retriever_extra}
\end{figure}

==> non-alternative-adaptive.tex <==

% \algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%

% \begin{figure}[t]\vspace{-1em}
% \begin{algorithm}[H]
% \caption{Non-Alternate Adaptive Retrieval } \label{alg: main}
% \begin{algorithmic}
% \Require Query $q$, initial ranking $R_0$, batch size $b$, budget $c$, graph $G$, top re-ranked documents $s$
% \Ensure Re-Ranked pool $R_1$
% \State $R_1 \gets \emptyset$ \Comment{Re-Ranking results}
% \State $F \gets \emptyset$ \Comment{Graph frontier}
% \State $S \gets \emptyset$ \Comment{top ranked documents}
% \State $B \gets$ \Call{Score}{top $b$ from $R_0$, subject to $c$} \Comment{Using monoT5}
% \State $R_1 \gets R_1 \cup B$ \Comment{Add batch to results}
% % \State\HiLi $\Call{SetAff}{.} \gets 0$ \Comment{Initialize expected affinity scores}
% \Do

%   \State $S \gets$ \Call{Select}{top $s$ from $R_1$} \Comment{Select top $s$ ranked docs}
%   \State $F \gets F \cup (\Call{Neighbours}{B \cap S, G} \setminus R_1$) \Comment{Update frontier}
% % \State\HiLii $\Call{SetAff}{d} \gets \Call{SetAff}{d} + \Call{SetAff}{d,R_1}, \quad \forall d \in F$ \Comment{\small{Update Exp. Aff. Scores using (\ref{eq:eaffm})}}
% % \normalsize
% \State $F \gets \Call{InterSetAff}{q, d,S} \quad \forall d \in F$ \Comment{Assign interpolated set affinity scores}
% \State $B \gets$ \Call{Score}{top $b$ from $F$, subject to $c$} \Comment{Using monoT5}
% \State $R_1 \gets R_1 \cup B$ \Comment{Add batch to results}
% \State $F \gets F \setminus B$ \Comment{Discard batch from frontier}


% \doWhile{$|R_1| < c$}
% %\State $R_1 \gets R_1 \cup \Call{Backfill}{R_0, R_1}$ \Comment{Backfill remaining items}
% \end{algorithmic}
% \end{algorithm} %\vspace{-2em}
% \end{figure}


% \begin{figure}[t]\vspace{-1em}
% \begin{algorithm}[H]
% \caption{Bandit-based Adaptive Retrieval } \label{alg: main}
% \begin{algorithmic}
% \Require Query $q$, initial ranking $R_0$, batch size $b$, budget $c$, top re-ranked documents $s$
% \Ensure Re-Ranked pool $R_1$
% \State $U \gets \emptyset$ \Comment{Re-Ranking results}
% \State $F \gets \emptyset$ \Comment{Graph frontier}
% \State $S \gets \emptyset$ \Comment{top ranked documents}
% \State $B \gets$ \Call{Score}{top $b$ from $R_0$, subject to $c$} \Comment{Using monoT5}


% % \State\HiLi $\Call{SetAff}{.} \gets 0$ \Comment{Initialize expected affinity scores}
% \Do

%   \State $S \gets$ \Call{Select}{top $s$ from $R_1$} \Comment{Select top $s$ ranked docs}

%   \State $X \gets UNROLL(S)$ (get n-hop neighbors of top-s documents)

%   \State $U_t \gets CASE(X \cup B)$

%   \State $R_1 \gets R_1 \cup U_t$ \Comment{Add batch to results}
  
 % \State $F \gets F \cup (\Call{Neighbours}{B \cap S, G} \setminus R_1$) \Comment{Update frontier}
% \State\HiLii $\Call{SetAff}{d} \gets \Call{SetAff}{d} + \Call{SetAff}{d,R_1}, \quad \forall d \in F$ \Comment{\small{Update Exp. Aff. Scores using (\ref{eq:eaffm})}}
% \normalsize

%\State $B \gets$ \Call{Score}{top $b$ from $F$, subject to $c$} \Comment{Using monoT5}
%\State $R_1 \gets R_1 \cup B$ \Comment{Add batch to results}
% \State $R_0 \gets R_0 \setminus B$ \Comment{Discard batch from frontier}


% \doWhile{$|R_1| < c$}
% %\State $R_1 \gets R_1 \cup \Call{Backfill}{R_0, R_1}$ \Comment{Backfill remaining items}
% \end{algorithmic}
% \end{algorithm} %\vspace{-2em}
% \end{figure}

==> plots/ar_plots.tex <==

\begin{figure}
    \centering
    \begin{subfigure}{0.48\columnwidth}
        \centering
    \begin{tikzpicture}
		\begin{axis}[
			width =  1.2\linewidth,
			height =1.0\linewidth,
			major x tick style = transparent,
			grid = major,
		    grid style = {dashed, gray!20},
			xlabel = {\#batches scored by CE},
			ylabel = {Recall@100},
			title={\small{Adaptive Retrieval}},
            title style={yshift=-1.5ex}, % Shift title closer to the plot
            symbolic x coords={0, 1,2,3,4,5,6,7},
            xtick={0,1,2,3,4,5,6,7},
            xtick distance=20,
            enlarge x limits=0.05,
            xlabel near ticks,
            ylabel near ticks,
            % ymax=0.65,
            ymin=0.45,
            % every axis x label/.style={at={(0.5, -0.08)},anchor=near ticklabel},
            every axis y label/.style={at={(-0.18, 0.5)},rotate=90,anchor=near ticklabel},
			]

	\addplot [color=black, style= dashed, line width = 1.0pt] table [x index=0, y index=1, col sep = comma] {plots/ablation/intro.txt}
        node[pos=0.5, anchor=west, yshift=2pt, below] {BM25};
			
	\addplot [color=black, line width = 1.0pt] table [x index=0, y index=2, col sep = comma] {plots/ablation/intro.txt}node[pos=0.7, sloped, below] {\sys{}};

   	\addplot [color=black, line width = 1.0pt] table [x index=0, y index=3, col sep = comma] {plots/ablation/intro.txt}
    node[pos=0.7, sloped, below] {\quamsys{}};

   	\addplot [color=red, line width = 1.0pt] table [x index=0, y index=4, col sep = comma] {plots/ablation/intro.txt}
    node[pos=0.5, sloped, yshift=5pt, above] {\cerberus{}};
   
    \end{axis}
    \end{tikzpicture}    
    \caption{ } 
    \label{fig:adaptive_cross_enc_call_vs_perf}
    \end{subfigure} 
    \hspace{0.02\columnwidth}
    %\hfill
    \begin{subfigure}{0.48\columnwidth}
        \centering
    \begin{tikzpicture}
		\begin{axis}[
			width =  1.2\linewidth,
			height = 1.0\linewidth,
			major x tick style = transparent,
			grid = major,
		    grid style = {dashed, gray!20},
			xlabel = {\#batches scored by CE},
			ylabel = {Error},
			title={\small{Adaptive Retrieval}},
            title style={yshift=-1.5ex}, % Shift title closer to the plot
            symbolic x coords={1,2,3,4,5,6,7},
            xtick={1,2,3,4,5,6,7},
            xtick distance=20,
            enlarge x limits=0.05,
            xlabel near ticks,
            ylabel near ticks,
            % every axis x label/.style={at={(0.5, -0.08)},anchor=near ticklabel},
            every axis y label/.style={at={(-0.09, 0.5)},rotate=90,anchor=near ticklabel},
			]


   	\addplot [color=red, line width = 1.0pt] table [x index=0, y index=4, col sep = comma] {plots/ablation/ar_cross_enc_vs_error.txt}
    node[pos=0.7, yshift=5pt, above] {\cerberus{}};
   
        \end{axis}
    \end{tikzpicture}  

    \caption{ } 
    \label{fig:adaptive_error}
    \end{subfigure} 
    \vspace{-2em}
    \caption{Recall (left) and estimation error (right) comparison on the \textbf{TREC DL19} dataset for adaptive retrieval, for ranking budget of 100 and batch of size 16.}
    \label{fig:ar_plots}    
    \vspace{-1.8em}
    \Description{}
\end{figure}
 % when the number of batches scored by cross-encoder varies for \cerberus{} 

==> plots/ar_time.tex <==

% \begin{tikzpicture}
% % \edef\mylst{"69.37","48.82","76.78","54.75"}
% % \edef\explora{"79.07","53.94","79.65","59.46"}
% \edef\mylst{"","","","",""}
% \edef\explora{"","","","",""}

%     \begin{axis}[
%             ybar=5pt,
%             width =  1.2\linewidth,
% 			height =0.9\linewidth,
%             bar width=0.25,
%             every axis plot/.append style={fill},
%             grid=major,
%             xtick={1, 2, 3},
%             xticklabels={0.51 $\pm$ 0.56 $\pm$ 0.1, 0.59 $\pm$ 0.1},
%             xlabel={Recall@100},
%             ylabel style = {font=\small},
%         yticklabel style = {font=\boldmath \tiny,xshift=0.5ex},
%         xticklabel style ={font=\small,yshift=0.5ex},
%             ylabel={time},
%             enlarge x limits=0.25,
%             ymin=0,
%             ymax=0.7,
%             legend style ={font=\small,yshift=0.5ex},
%             area legend,
%             nodes near coords style={font=\tiny,align=center,text width=2em},
%             legend entries={RRF, \cerberus{}},
%             legend cell align={left},
%             legend pos=north west,
%             legend columns=-1,
%             legend style={/tikz/every even column/.append style={column sep=0.5cm}},r_
%         \addplot+[
%             ybar,
%             plotColor3*,
%             nodes near coords=\pgfmathsetmacro{\mystring}{{\mylst}[\coordindex]}\textbf{\mystring},
%             nodes near coords align={vertical},
%             draw=black,
%             postaction={
%                     pattern=north east lines
%                 },
%         ] plot coordinates {
%                 (1,0.604)
%                 (2,0.604)
%                 (3,0)
%                 (4,0)
%                 (5,0)
%             };
%         \addplot+[
%             ybar,
%             plotColor1*,
%             draw=black,
%             nodes near coords=\pgfmathsetmacro{\mystring}{{\explora}[\coordindex]}\textbf{\mystring},
%     nodes near coords align={vertical},
%             postaction={
%                     pattern=north west lines
%                 },
%         ] plot coordinates {
%                 (1,0.636)
%                 (2,0.647)
%                 (3,0)
%                 (4,0)
%                 (5,0)
%             };

%                     \addplot+[
%             ybar,
%             plotColor4*,
%             draw=black,
%             nodes near coords=\pgfmathsetmacro{\mystring}{{\explora}[\coordindex]}\textbf{\mystring},
%     nodes near coords align={vertical},
%             postaction={
%                     pattern=north west lines
%                 },
%         ] plot coordinates {
%                 (1,0.636)
%                 (2,0.647)
%                 (3,0)
%                 (4,0)
%                 (5,0)
%             };
 

%     \end{axis}

% \end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    width=1.2\linewidth,
	height = 0.9\linewidth,
    ybar=0.9,
    bar width=5.0, % Set the width of the bars here
    enlargelimits=0.15,
    title={},
    legend style={at={(0.5,-0.15)},
      anchor=north,legend columns=-1},
    ylabel={time},
    ylabel near ticks,
    xlabel={Recall@100},
    every axis y label/.style={at={(-0.10, 0.5)},rotate=90,anchor=near ticklabel},
    symbolic x coords={50,100, 1000},
    xtick=data,
    yticklabel style = {xshift=0.5ex},
    xticklabel style = {yshift=0.5ex},
    nodes near coords={},
    nodes near coords align={vertical},
    legend columns=4,
    legend entries={BM25>>MonoT5;,\sys{BM25};, \sys{BM25}+\laff;,\quamsys{BM25}},
    legend to name=compdl19,
    enlarge x limits=0.25]


\addplot[fill=black!60] coordinates {(50,0.389) (100,0.497) (1000,0.755495)};
\addplot[pattern=north west lines, pattern color=blue!60] coordinates {(50,0.426) (100,0.547) (1000,0.833)};
\addplot[pattern=north east lines, pattern color=red!60] coordinates {(50,0.451) (100,0.600) (1000,0.861)};
\addplot [fill=blue!60] coordinates {(50,0.480) (100,0.611) (1000,0.867)};

\end{axis}
\end{tikzpicture}


==> plots/hybrid_plots.tex <==

\begin{figure}
    \centering
    \begin{subfigure}{0.48\columnwidth}
        \centering
 \begin{tikzpicture}
		\begin{axis}[
			width =  1.2\linewidth,
			height =1.\linewidth,
			major x tick style = transparent,
			grid = major,
		    grid style = {dashed, gray!20},
			xlabel = {\#batches scored by CE},
			ylabel = {Recall@100},
			title={\small{Hybrid Retrieval}},
            title style={yshift=-1.5ex}, % Shift title closer to the plot
            symbolic x coords={0,1,2,3,4,5,6,7},
            xtick={0, 1,2,3,4,5,6,7},
            xtick distance=20,
            enlarge x limits=0.05,
            xlabel near ticks,
            ylabel near ticks,
            % every axis x label/.style={at={(0.5, -0.08)},anchor=near ticklabel},
            ymax=0.69,
            every axis y label/.style={at={(-0.18, 0.5)},rotate=90,anchor=near ticklabel},
			]

	% \addplot [color=black, style= dashed, line width = 1.0pt] table [x index=0, y index=1, col sep = comma] {plots/ablation/crossenc_vs_perf_hybrid.txt}
 %        node[pos=0.5, anchor=west, yshift=7pt] {BM25};
			
	\addplot [color=black, line width = 1.0pt] table [x index=0, y index=2, col sep = comma] {plots/ablation/crossenc_vs_perf_hybrid.txt}node[pos=0.7, sloped, above] {RRF};

   	\addplot [color=black, line width = 1.0pt] table [x index=0, y index=3, col sep = comma] {plots/ablation/crossenc_vs_perf_hybrid.txt}
    node[pos=0.5, sloped, above] {CC};


   	\addplot [color=red, line width = 1.0pt] table [x index=0, y index=4, col sep = comma] {plots/ablation/crossenc_vs_perf_hybrid.txt}
    node[pos=0.7, yshift=5pt, above] {\cerberus{}};
   
    \end{axis}
    \end{tikzpicture}    
    \caption{} 
    \label{fig:hybrid_cross_enc_vs_perf}
    \end{subfigure} 
    \hspace{0.02\columnwidth}
   % \hfill
    \begin{subfigure}{0.48\columnwidth}
        \centering
    \begin{tikzpicture}
		\begin{axis}[
			width =  1.2\linewidth,
			height =1.0\linewidth,
			major x tick style = transparent,
			grid = major,
		    grid style = {dashed, gray!20},
			xlabel = {\#batches scored by CE},
			ylabel = {Error},
			title={\small{Hybrid Retrieval}},
            title style={yshift=-1.5ex}, % Shift title closer to the plot
            symbolic x coords={1,2,3,4,5,6,7},
            xtick={1,2,3,4,5,6,7},
            xtick distance=20,
            enlarge x limits=0.05,
            enlarge y limits=0.08,
            xlabel near ticks,
            ylabel near ticks,
            %ymax=0.8,
            % every axis x label/.style={at={(0.5, -0.08)},anchor=near ticklabel},
            every axis y label/.style={at={(-0.08, 0.5)},rotate=90,anchor=near ticklabel},
			]

	% \addplot [color=black, style= dashed, line width = 1.0pt] table [x index=0, y index=1, col sep = comma] {plots/ablation/intro.txt}
 %        node[pos=0.5, anchor=west, yshift=7pt] {BM25};
			
	% \addplot [color=black, line width = 1.0pt] table [x index=0, y index=2, col sep = comma] {plots/ablation/intro.txt}node[pos=0.7, sloped, above] {\sys{}};

 %   	\addplot [color=black, line width = 1.0pt] table [x index=0, y index=3, col sep = comma] {plots/ablation/intro.txt}
 %    node[pos=0.5, sloped, above] {\quamsys{}};

   	\addplot [color=red, line width = 1.0pt] table [x index=0, y index=4, col sep = comma] {plots/ablation/cross_enc_vs_error.txt}
    node[pos=0.7, yshift=5pt, sloped, above] {\cerberus{}};
   
        \end{axis}
    \end{tikzpicture}    
    \caption{ } 
    \label{fig:hybrid_error}
    \end{subfigure} 
    \vspace{-2em}
    \caption{Recall (left) and estimation error (right) comparison for hybrid retrieval setting on the \textbf{TREC DL19} dataset when the number of batches of scored by cross-encoder (CE) varies for \cerberus{} for ranking budget of 100 and batch of size 16.}
    \label{fig:hybrid}    
    \Description{}
    \vspace{-1.0em}
\end{figure}


==> plots/latency.tex <==

\begin{figure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
        \centering
    \begin{tikzpicture}
    \begin{axis}[
    width =  1.4\linewidth,
	height =1.2\linewidth,
	major x tick style = transparent,
	grid = major,
	grid style = {dashed, gray!20},
    ybar=0.9,
    bar width=6.0, % Set the width of the bars here
    enlargelimits=0.15,
    title style={yshift=-1.5ex}, % Shift title closer to the plot
    legend style={at={(0.20,.88)},
       anchor=north,legend columns=-1, font=\tiny},
    ylabel={},
    xlabel={Recall@100},
    title={\small{time (ms/query)}},
    every axis y label/.style={at={(-0.00, 0.5)},rotate=90,anchor=near ticklabel},
    symbolic x coords={0.51,0.56, 0.59},
    xtick={0.51,0.56, 0.59},
    %yticklabel style = {xshift=0.5ex},
    %xticklabel style = {yshift=0.5ex},
    nodes near coords={},
    nodes near coords align={vertical},
    ylabel near ticks,
    xlabel near ticks,
    yticklabel style = {font=\small,xshift=0.5ex},
    xticklabel style = {font=\small,yshift=0.5ex},
    %ymax=300,
    legend columns=1,
    legend entries={\sys{},\quamsys{},\cerberus{} },
    enlarge x limits=0.25]

\addplot[fill=gray!50] coordinates {(0.51, 68 ) (0.56,238) (0.59,276)};
\addplot[fill=blue!20] coordinates {(0.51, 65) (0.56, 130 ) (0.59,194 )};
\addplot[fill=red!30] coordinates {(0.51, 63) (0.56,102 ) (0.59, 178)};

\end{axis}
\end{tikzpicture}
    \caption{} 
        \label{fig:latency_adaptive_bars}
    \end{subfigure} 
    \hfill
    \hspace{-1cm}
    \begin{subfigure}{0.45\columnwidth}
        \centering
    \begin{tikzpicture}
    \begin{axis}[
    width =  1.4\linewidth,
	height =1.2\linewidth,
	major x tick style = transparent,
	grid = major,
	grid style = {dashed, gray!20},
    ybar=0.9,
    bar width=6.0, % Set the width of the bars here
    enlargelimits=0.15,
    legend style={at={(0.20,0.88)},
       anchor=north,legend columns=1, font=\tiny},
    ylabel={},
    xlabel={Budget $c$},
    title={\small{time (ms/query)}},
    title style={yshift=-1.5ex}, % Shift title closer to the plot
    every axis y label/.style={at={(0.15, 0.5)},rotate=90,anchor=near ticklabel},
    symbolic x coords={50,100, 250},
    xtick={50,100, 250},
    %yticklabel style = {xshift=0.5ex},
    %xticklabel style = {yshift=0.5ex},
    nodes near coords={},
    nodes near coords align={vertical},
    ylabel near ticks,
    xlabel near ticks,
    yticklabel style = {font=\small,xshift=0.5ex},
    xticklabel style = {font=\small,yshift=0.5ex},
    %ymax=650,
    legend columns=1,
    legend entries={CE ,Fit, Lookup},
    enlarge x limits=0.25]


\addplot[fill=black!60] coordinates {(50, 144.7 ) (100,259) (250,601.7)};
\addplot[fill=purple!20] coordinates {(50, 4.5) (100, 9.18 ) (250,22.9 )};
\addplot[fill=yellow!30] coordinates {(50, 4.9) (100,11.25 ) (250, 32.2)};

\end{axis}
\end{tikzpicture}
    \caption{} 
        \label{fig:latency_cereberus_comp}
    \end{subfigure} 
    \label{fig:latency}  
    \vspace{-1.em}
    \caption{Computational efficiency of our proposed methods \cerberus{} in comparison to adaptive retrieval approaches (left) and overheads from different components (right) during online relevance estimation.}
    \vspace{-2em}
    \Description{}
\end{figure}


==> prompt-intents.tex <==
\begin{tcolorbox}[title=\textbf{LLM Prompt}: Intent candidate generation]
\small
A person wants to find out distinct intention behind the question \textbf{\{query\}}. Give five descriptive (max. 15 words) distinct intentions which are easy to understand. Consider all documents in your response. Response should be in this format:

\textbf{Intention}:: <intention> , \textbf{Doc\_list}::<list of documents with the intention> \\ \textbf{Documents}: \textbf{\{list of input documents\}}
\end{tcolorbox}


==> results.tex <==
\section{Results Analysis}
\label{sec:results}

The primary results for the effectiveness analysis of our experiments are shown in Table \ref{tab:main}. We discuss the results in detail in the following sections.
\input{plots/hybrid_plots}

\subsection{Effectiveness of \cerberus{}}
To answer \textbf{RQ1}, we evaluate \cerberus{} on TREC DL 19, 20 (Table \ref{tab:main}) and TREC DL 21, 22 (Table \ref{tab:msmarco-v2}). We compare \cerberus{} with existing state-of-the-art methods in hybrid and adaptive retrieval setups.

\subsubsection{Adaptive Retrieval}: We compare \cerberus{} to state-of-the-art adaptive retrieval methods \gar{} and \quam{} to answer \textbf{RQ 1}. We observe that \cerberus{} outperforms existing approaches, as indicated by Recall@c for different retrieval budgets with significant gains at lower budgets. On DL21, we observe that \cerberus{} advances Recall@50 to \textbf{0.406} providing gains of \textbf{30.55 \%} over \quam{} and \textbf{22.66 \%} over \gar{}. We also observe that \cerberus{} advances Recall@50 from 0.460 (\quam{}), 0.417 (\gar{}) to 0.514 (\textbf{11.74\%} and \textbf{23.26\%} respectively) on DL19.  We observe that this primarily stems from the principled selection of documents for adaptive scoring by \cerberus{}. The existing adaptive retrieval methods like \gar{} and \quam{} alternate between the first-stage retrieval results and neighborhood list till the budget constraint is satisfied. \cerberus{} departs from this heuristic by estimating the utility (\textsc{EstRel}) of the documents online through an inexpensive approach, as detailed in Section \ref{sec:estimated rel}. This results in the balanced exploitation of documents from first-stage retrieval with sufficient exploration of the neighborhood of documents already scored by the expensive ranker. This leads to the prioritization of relevant documents that may have low first-stage retrieval scores but high utility as measured by our proposed relevance estimation approach. Surprisingly, we also observe that \cerberus{} outperforms the exhaustive retrieval pipeline, which employs the expensive scorer to score all documents in the corpus without first-stage retrieval.  This further casts light on the ability of the estimated utility in \cerberus{} to reduce noisy documents in the search space and prioritize potentially relevant documents.


\subsubsection{Hybrid Retrieval:} The hybrid retrieval results are as shown in Table~\ref{tab:main} and~\ref{tab:msmarco-v2}. We observe that \cerberus{} provides statistically significant performance gains over existing rank fusion based hybrid retrieval approaches, namely RRF and CC. From Table \ref{tab:msmarco-v2}, we observe impressive gains, where \cerberus{} outperforms CC by \textbf{11.74 \%} and RRF by \textbf{17.12\%} for Recall@100 on DL21. We also observe that \cerberus{} advances Recall@100 on DL22 by \textbf{7.46 \%}, when compared to CC  and by \textbf{14.09\%} when compared to RRF. We also observe that \cerberus{} significantly improves Recall@50 from 0.489 to 0.558 (\textbf{14.11 \%}), 0.513 (RRF) to 0.558 (\textbf{8.9\%}).

We observe a similar trend in Recall in different budgets, with \cerberus{} providing statistically significant gains.  These performance gains primarily stem from the adaptive nature of the \cerberus{} which prioritizes the documents to be scheduled for scoring. In contrast to traditional fusion-based hybrid retrieval methods that pick top-k documents from merged list while ignoring remaining documents. Since the search space comprises documents with low retrieval scores which might be relevant, it is critical to capture these documents and prioritize them for scoring. \cerberus{} exploits the explore-exploit paradigm from Multi-Arm Bandits (MAB) to achieve the prioritization of such documents. It tries to balance the exploitation of documents with high retrieval scores (Q2DAff) with exploration of potentially relevant documents that have high affinity to scored documents (D2DAff).



\mpara{Insight 1:} \cerberus{} achieves high recall in hybrid retrieval and adaptive retrieval settings by dynamically learning to prioritize documents through inexpensive estimation/approximation of document relevance scores.  



\subsection{Significance and Quality of Estimated Utility.}
\label{sec:rq-2}

While the overall performance indicates that the proposed utility estimation aids in the prioritization of documents it does not shed light on it's absolute quality and ability to serve as a proxy for the score from the expensive ranker.

Since the utility computed for documents online (\textsc{EstRel}) forms the cornerstone of \cerberus{}, to answer \textbf{RQ3}, we analyze the quality of scores estimated online. 

\input{tables/main_results}
\noindent \textbf{Adaptive Retrieval:}
Similarly for adaptive retrieval, we plot the error in estimated utility in Figure \ref{error:adaptive}. We observe a trend akin to a hybrid retrieval setup. We observe that the error slowly decreases, as $cb$ increases with a sharp drop for full ranker budget $cb=7$ setting, as more samples are scored.


We also plot ranker budget vs Recall@100 for DL19. We observe from the resulting Figure \ref{fig:adaptive_cross_enc_call_vs_perf} at all  ranker budgets ($cb$) consistently outperforms state-of-the-art adaptive retrieval methods like \gar{} and \quam{}. In particular, we observe that even at $cb=1$, \cerberus{} provides superior performance where the utility is employed as proxy to score documents instead of calls to the expensive ranker. This indicates the quality of the estimated utility scores that aid in prioritizing relevant document through principle exploration. We also posit that this phenomenon is also due to heuristic document selection of \gar{} and \quam{} which alternates between initial list and neighborhood of documents. At lower ranker budgets, \gar{} and \quam{} scores limited documents and backfills the rest of the documents till $c$ is satisfied using scores from initial ranked list. In contrast, the learned utility estimator in \cerberus{} performs a principled exploration of initial results and the new neighbors to prioritize documents for each batch till $c$ is reached.

 \noindent \textbf{Hybrid Retrieval:}
To demonstrate the quality of estimated scores in the hybrid retrieval setup, we first analyze the error between the estimated relevance (utility \textsc{EstRel}) and the actual relevance score from the ranker for different cross encoder budgets. Here, cross encoder budget $cb$ refers to number of samples that are allowed to be ranked and $cb\le
c$. The plot for hybrid retrieval with $c=100$ and $b=16$ for different cross- encoder budgets $cb=\{1...7\}$ is shown in Figure \ref{fig:hybrid_error}. For instance, at $cb=2$ only 32 samples are scored and used to learn parameters for utility estimation which are then employed to estimate utility for the rest of the  documents till the budget $c$ is satisfied. We observe that at $cb=1$, the error is high as in the first iteration parameters are initialized randomly resulting in the utility (EstRel) being poor estimates of actual relevance. However, at $cb=2$, we observe a sharp decline in error indicating that the utility closely approximates the actual relevance scores from the ranker. We observe that the error slowly decreases, as $cb$ increases, as more samples are scored. This phenomenon primarily as the estimator procures more samples to learn from resulting in better utility estimation. The quality of estimated utility is also evident from Figure  
\ref{fig:hybrid_cross_enc_vs_perf}, where when only 16 documents are scored, \cerberus{} already outperforms RRF and CC by estimating high quality utility scores for the remainder of the documents.



\mpara{Insight 2:} Online relevance/utility estimation of \cerberus{} works well across hybrid and adaptive retrieval settings and closely approximates actual relevance estimates from the  ranker.
 \subsection{Sample Efficiency of \cerberus{}}

 To answer \textbf{RQ3}, we demonstrate the latency and sample efficiency gains provided by \cerberus{} over \gar{} and \quam{} in adaptive retrieval setting. 
 In Figure~\ref{fig:latency_bars}, we record the time taken by \cerberus{} and contemporary adaptive retrieval methods for attaining specific recall performance. In particular, we observe that to reach a Recall@100 of 0.56, \cerberus{} requires only 2 ranker/cross-encoder calls (\textbf{102 ms/query}) providing a speedup of \textbf{2$\times$}  compared to \gar{} that takes 8 calls with \textbf{238 ms / query}. This demonstrates that \cerberus{} requires fewer scored samples to attain higher recall owing to the efficient online relevance estimation. From Table \ref{tab:latency-ranklamma}, we observe that \cerberus{} provides competitive or better performance than existing adaptive retrieval methods in terms of latency and Recall@c when employing an expensive ranker like RankLLaMa. We observe that \cerberus{} provides speedups of \textbf{2x-3x} on average and upto \textbf{9 $\times$} for $c=1000$ at different budgets compared to \gar{} and \quam{}. This is primarily a result of sample efficient nature of \cerberus{} which requires less number of scored samples to estimate utility scores for rest of documents that serves as proxy for actual relevance scores. 
 
\mpara{Insight 3:} \cerberus{} is sample efficient when compared to state-of-the-art adaptive retrieval methods requiring fewer documents to be scored by the expensive ranker on average. it provides speedups of upto \textbf{2$\times$} for standard rankers like MonoT5 and \textbf{7 $\times$} for more expensive LLM based rankers like RankLLaMa.

% \begin{table*}
%     \centering
%     \caption{Effectiveness of \gar{} and \quam{}  on TREC DL19 and 20 dataset. Significant improvements (paired t-test, $p<0.05$, using Bonferroni correction) with the re-ranking baseline (retriever>>MonoT5) and \gar{} are marked with $B$ and $G$ respectively in the superscript. The best result for each pipeline is in bold. }
%     {\small
%     \setlength{\tabcolsep}{4.5pt}
%     %\hskip-4.0cm
%     \begin{tabular}{llrrrrrrrrr}

% \toprule
% \multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{3}{c}{$c=50$}&\multicolumn{3}{c}{$c=100$}&\multicolumn{3}{c}{$c=1000$} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
% Dataset&Pipeline  & nDCG@10 & nDCG@c & Recall@c & nDCG@10 & nDCG@c  & Recall@c & nDCG@10 & nDCG@c & Recall@c\\
% \midrule
% \rowcolor{gray!70}
% \multirow{11}{*}{\textbf{DL19}} \cellcolor{white}& MonoT5-Exh.   & 0.672 & 0.625& 0.512  & 0.672 & 0.611  & 0.599 &0.672 & 0.691 & 0.834  \\
% \cmidrule{2-11}
% \rowcolor{gray!50}
% \cellcolor{white} &BM25>>MonoT5   &  0.676 & 0.546 &0.389 & 0.696 & 0.571 & 0.497 & 0.724  &0.696&  0.755  \\
%   & \idnt w/ \sys{BM25}   &  0.694 & 0.573  & 0.426  & 0.716  & 0.605  & 0.547  & 0.719 & 0.736 & ${}^{B}$0.833\\
%  & \idnt w/ \quamsys{BM25} & \bf0.706 & ${}^{BG}$\bf0.615 & ${}^{BG}$\bf0.480  & \bf0.720& ${}^{BG}$\bf0.651 & ${}^{BG}$\bf0.611  & \bf0.732 & ${}^{B}$\bf0.758  & ${}^{BG}$\bf0.867\\

% \cmidrule{3-11}
%  & \idnt w/ \sys{TCT}   & \bf0.724   & ${}^{B}$\bf0.620  & ${}^{B}$0.476   & ${}^{B}$\bf0.747  &  ${}^{B}$\bf0.656 & ${}^{B}$\bf0.606 &  \bf0.734  & ${}^{B}$\bf0.754 &   ${}^{B}$\bf0.859 \\
%  & \idnt w/ \quamsys{TCT} & 0.704 & ${}^{B}$0.612 & ${}^{B}$\bf0.481   & 0.722& ${}^{B}$0.642 & ${}^{B}$0.601&0.721& ${}^{B}$0.747  & ${}^{B}$0.857  \\ 


% \bottomrule
% \end{tabular}
% }
% \label{tab:main}
% \end{table*}








\input{tables/msmarco-v2}



% \begin{table*}
%     \centering
%     \caption{Multi-Arms-Bandit results}
%     \begin{tabular}{lccc}
%         \toprule
%         & \multicolumn{3}{c}{$c=100$}  \\
%          \cmidrule{2-4}
%         pipeline& nDCG@10 &nDCG@c  &Recall@c \\
%         \midrule
%          BM25 & 0.499 &  0.503  & 0.497 \\
%         BM25>>MonoT5  &0.696 & 0.571&  0.497\\
%         \idnt w/ \sys{BM25} & 0.716&  0.605&  0.547 \\
%         \idnt w/ \cerberussys{BM25} & 0.699 &0.602& 0.567 \\
%         \idnt w/ \cerberussys{BM25}+\laff & 0.705 &0.629& 0.594 \\

%         \bottomrule
%     \end{tabular}
%     \label{tab:mab}
% \end{table*}



==> tables/efficiency-mono-t5.tex <==
\newcommand{\gt}[1]{\tiny{(\tikz\draw[green!60!black, fill=green!60!black] (0,0) -- (0.10,0) -- (0.05,0.10) -- cycle;{#1\%}})}

\newcommand{\rt}[1]{\tiny{(
    \tikz\draw[red, fill=red] (0,0) -- (0.10,0) -- (0.05,-0.10) -- cycle;%
    {#1\%})}}

\begin{table*}
\centering
\caption{Mean re-ranking latency per query (in ms) at different re-ranking budgets using MonoT5 and RankLLaMA rerankers when the first-stage retrieval of different budgets ($c$) is done using BM25. The number of batches re-ranked by ranker \cerberus{} is enclosed in braces. }
\vspace{-1.5em}
\label{tab:latency}
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{clllccc|lllccc}
\toprule
& \multicolumn{6}{c|}{MonoT5}& \multicolumn{6}{c}{RankLLaMA}  \\
\cmidrule{2-7}\cmidrule{8-13}
&  \multicolumn{3}{c}{time (ms/query)}& \multicolumn{3}{c|}{Recall@c} &\multicolumn{3}{c}{time (ms/query)}& \multicolumn{3}{c}{Recall@c}  \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 

c   & \sys{} & \quamsys{}  & \cerberussys{} &\sys{}  & \quamsys{} & \cerberussys{}  & \sys{} & \quamsys{}  & \cerberussys{} &\sys{}  & \quamsys{} & \cerberussys{}\\
\midrule
50    & 179.92  & 173.21  & 125.91(2)    & 0.417 & 0.460  & \textbf{0.500} &6269.77   &6027.12   &  3925.54(2)   & 0.421 & 0.449 & \textbf{0.492} \\
100    & 356.53  &328.82  & 272.04(4)    &  0.539 &0.594   & 0.594 & 12746.55  &12074.67  & 7830.41(4)    & 0.542  & \textbf{0.600}  & \textbf{0.600} \\
250     &877.19 &816.90 &599.24(8)   & 0.692 & 0.745  &0.715 & 32312.97 & 30539.78 &  16092.16(8) & 0.684 &0.761  &  0.719\\
% 500    &   &   &   &   & 0. & 0.  &  \\
% 750  &   &    &   &   & 0. & 0.  &  \\
\multirow{2}{*}{1000}    &  3418.98 & 3219.45  & 1848.26(8)  & 0.836 &0.874  & 0.827  & 127617.45  & 120885.39   & 16327.25(8) & 0.854 &0.881 & 0.829 \\
&   &   &  2188.29(16)  &  &  & 0.841  &   &   & 31939.78(16) & &  & 0.853 \\

\bottomrule
\end{tabular}
\vspace{-1.em}
\end{table*}




==> tables/efficiency-rank-llama.tex <==

\begin{table*}
\centering
\caption{Mean re-ranking latency per query (in ms) at different re-ranking budgets using RankLLaMA (pointwise ranker). The number of ranker calls (or number of batches) is enclosed in braces for \cerberus{}.  }
\label{tab:latency-ranklamma}
\begin{tabular}{rrclccclll}
\toprule
& &\multicolumn{3}{c}{time (ms)}& \multicolumn{3}{c}{Recall@c}  \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} 
c & $|S|$  & \sys{BM25} & \quamsys{BM25}  & \cerberussys{BM25} &\sys{BM25}  & \quamsys{BM25} & \cerberussys{BM25} \\
\midrule
50   & &6269.77   &6027.12   &  3925.54(2)   & 0.421 & 0.449 & \textbf{0.492} \\
\cmidrule{3-8}
\multirow{2}{*}{100}   & & 12746.55  &12074.67  & 5833.90(3)    & 0.542  & \textbf{0.600}  &0.581 \\
   & &   &  & 7830.41(4)    &   &   & \textbf{0.600}\\
%   & &  &  & (4)    &   &   &  \\
\cmidrule{3-8}
% 250   &  &  &  &  (3) & 0.684 &0.761  &0.667  \\
250   &  & 32312.97 & 30539.78 &  16092.16(8) & 0.684 &0.761  &  0.719\\
% 500    &   &   &   &   &  &   &  \\
% 750  &   &    &   &   &  &   &  \\
\cmidrule{3-8}
\multirow{3}{*}{1000}  &   & 127617.45  & 120885.39   & 16327.25(8) & 0.854 &0.881 & 0.829\\
 &   &   &  & 31939.78(16)  &    &  & 0.839   \\
 &   &   &  & 64390.74(32)  &    &  & 0.853   \\

\bottomrule
\end{tabular}
\end{table*}





==> tables/features.tex <==
\begin{table*}
    \centering
            \caption{Description of different features used for calculating relevance estimates. These features can be divided into two levels of affinity taxonomy, \textsc{Q2DAff} and \textsc{D2DAff}.}
    \vspace{-1em}
    \begin{tabular}{cccccll}
        \toprule
        Feature & Notation & Taxonomy &\multicolumn{2}{c}{Source} & Description & \\
         &   & & Offline & Online  & \\
        \midrule
        $x_1$ &  $BM25(q,d)$ & \textsc{Q2DAff}& &   \cmark&Lexical similarity between query and document. \\
        $x_2$ & $TCT(q,d)$ & \textsc{Q2DAff} & &   \cmark &Semantic similarity between query and document. \\
        $x_3$ & $RM3(q^\prime, d)$&\textsc{D2DAff} & &\cmark &Lexical similarity between expanded query using RM3 and document. \\
        $x_4$ & $BM25(d,d^\prime)$ &\textsc{D2DAff} & \cmark & & Lexical similarity between pair of documents. \\
        $x_5$ & $TCT(d,d^\prime)$ &\textsc{D2DAff} & \cmark& & Semantic similarity between pair of documents. \\
        $x_6$ & $\textsc{Laff}(d,d^\prime)$ & \textsc{D2DAff}& \cmark & & Learnt affinity or similarity between pair of documents~\cite{rathee2024quam}. \\
        \bottomrule
    \end{tabular}
    \label{tab:features}
    %\vspace{-1.5em}
\end{table*}

==> tables/hybrid_retrieval.tex <==


\begin{table*}
    \centering
    \caption{Effectiveness of hybrid retrieval results. }
    {\small
     \setlength{\tabcolsep}{4.5pt}
    \begin{tabular}{llrrrrrrrrr}
        \toprule
        \multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{3}{c}{$c=50$}&\multicolumn{3}{c}{$c=100$}&\multicolumn{3}{c}{$c=1000$} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
Dataset&Pipeline  & nDCG@10 & nDCG@c & Recall@c & nDCG@10 & nDCG@c  & Recall@c & nDCG@10 & nDCG@c & Recall@c\\
    \midrule
    \rowcolor{gray!70}
   \cellcolor{white}  & MonoT5-Exh &0.672  & 0.625 &0.512 & 0.611 & 0.599 &0.599 &0.672 & 0.691 & 0.834 \\
    \cmidrule{2-11}
    \rowcolor{gray!50}
\multirow{6}{*}{\textbf{DL19}}  \cellcolor{white} & BM25>>MonoT5 &0.681  & 0.541 &0.389 & 0.699 &0.563   &0.488&0.719 &0.697 &0.755  \\
     %  &  \bf\textsc{Alternating} & &  &  &  & \\
     &     \idnt w/ \sys{BM25}  & 0.689  & 0.565 & 0.417 & 0.716 &0.594 &0.539 &0.727 &0.742 &0.836 \\
       % &  \idnt w/ \sys{BM25}+Laff  &0.705  &0.596  &0.444  & 0.734 &0.643 &0.593 &0.735 &0.761 &0.870 \\
        &  \idnt w/ \quamsys{BM25}  & 0.698 &0.597  & 0.460 &0.729 &0.639& 0.594 &0.742 &0.770 &0.874 \\

       %   \cmidrule{2-11}
       % &  \idnt w/ \sys{TCT}   & 0.712  & 0.608 & 0.472 &  &  &\\
       %  & \idnt w/ \sys{TCT}+Laff   &0.706  &0.601  &0.456 &  & & \\
       %   & \idnt w/ \quamsys{TCT}  & 0.693 &0.599  & 0.466 &  &  &\\
      %   \cmidrule{2-11}
      % &  \bf\textsc{Non-Alternating} & &  &  &  & \\
      %  &  \idnt w/ \sys{BM25}   & 0.683 & 0.546 & 0.401 &0.689 &0.551 &0.496\\
      %  & \idnt w/ \sys{BM25}+Laff  &0.711  &0.615  &0.465 & 0.739&0.655 &0.626 \\
      %   & \idnt w/ \quamsys{BM25}  & 0.715 &0.628  & 0.491 &0.717 &0.632 &0.590\\
        %   &   \idnt w/ CERBERUS (half)  & 0. 706 &0.636  & 0.509 &0.725  & 0.653  & 0.640 & & & \\
        % &   \idnt w/ CERBERUS   & \textbf{0. 727}& \textbf{0.657}  & \textbf{0.532} &\textbf{0.733}  & \textbf{0.672}  & \textbf{0.649} & & & \\
          % &   \idnt w/ CERBERUS++ (half)  & 0.687 & \textbf{0.619}& \textbf{0.494} & 0.683 & 0.621 & \textbf{0.598}  \\

        &   \idnt w/ \cerberussys{BM25}   & \textbf{0.703} & \textbf{0.643}& \textbf{0.514} & 0.706 & \textbf{0.650} & \textbf{0.619} & 0.723 & 0.759 & \textbf{0.874} \\

 \cline{2-11}
         &   \idnt w/ \sys{TCT}   & 0.712 & 0.608 & 0.472 & 0.732 &0.642  &0.592  & 0.741 & 0.764 &0.859 \\
        &   \idnt w/ \quamsys{TCT}   &0.692 & 0.600 & 0.466 & 0.722 &0.635  &0.595  &0.742 &0.767 &0.880 \\
        &   \idnt w/ \cerberussys{TCT}  &0.695& \textbf{0.637} & \textbf{0.501}  & 0.720 &\textbf{0.654} & \textbf{0.612}  & \\
      %  \cmidrule{2-11}
       % &  \idnt w/ \sys{TCT}   &0.716  & 0.620 & 0.486 &  &  &\\
       %  & \idnt w/ \sys{TCT}+Laff  &0.716  &0.617  &0.478 &  &  & \\
       %   & \idnt w/ \quamsys{TCT}  & 0.703 &0.621  & 0.484 &  &   &\\
           

        \midrule
    \rowcolor{gray!70}
    \cellcolor{white} & MonoT5-Exh &0.649  & 0.592 &0.576 & 0.649 &0.593 &0.670 &0.649 &0.682 &0.852 \\
        \cmidrule{2-11} 
        \rowcolor{gray!50}
        \multirow{6}{*}{\textbf{DL20}}  \cellcolor{white}  & BM25>>MonoT5 &0.676 & 0.559 &0.478 &0.685 &0.581 &0.584  &0.720 &0.711  &0.807 \\
      % &  \bf\textsc{Alternating} & &  &  &  & \\
     &     \idnt w/ \sys{BM25}  & 0.690 & 0.577 & 0.496 & 0.703 &0.607 &0.617 &0.714 &0.750 &0.884 \\
       % &  \idnt w/ \sys{BM25}+Laff  &0.707 &0.607  &0.548  &0.716 &0.643 &0.665 &0.708 &0.753 &0.898 \\
        &  \idnt w/ \quamsys{BM25}  & 0.714 &0.615  & 0.556 & 0.717 &0.652  &0.678 &0.709 &0.756 &0.901 \\

       %   \cmidrule{2-11}
       % &  \idnt w/ \sys{TCT}   & 0. & 0. & 0. &  &  &\\
       %  & \idnt w/ \sys{TCT}+Laff   &0.  &0.  &0. &  & & \\
       %   & \idnt w/ \quamsys{TCT}  & 0. &0.  & 0. &  &  &\\
       %  \cmidrule{2-11}
      % & \bf \textsc{Non-Alternating} & &  &  &  & \\
     %   &  \idnt w/ \sys{BM25}   & 0.670 & 0.534 & 0.459 &0.702& 0.587& 0.601\\
     %   & \idnt w/ \sys{BM25}+Laff  &0.706  &0.597  &0.538 & 0.726& 0.648 &0.691 \\
     %    & \idnt w/ \quamsys{BM25}  & 0.713 &0.616 & 0.543 & 0.719 &0.648&0.684 \\
          % &   \idnt w/ CERBERUS (half)  & 0.696  &0.613  & 0.577 &0.699  & 0.654  & 0.705 & 0.  & & \\
          %           &   \idnt w/ CERBERUS   & 0. 694 &\textbf{0.642}  & \textbf{0.612} &0.707  & \textbf{0.663}  & \textbf{0.721} & & & \\

              % &   \idnt w/ CERBERUS++ (half)  & 0.672 &0.606  & \textbf{0.575} &0.668  & 0.621  & 0.684 & & & \\
              
        &   \idnt w/ \cerberussys{BM25}   & 0.684& \textbf{0.626}  & \textbf{0.596} &0.681  & 0.641  & \textbf{0.711} & 0.700& 0.757 & 0.892 \\
         \cline{3-11}
        &   \idnt w/ \sys{TCT}   &0.728 & 0.620 & 0.566 & 0.716 &0.648 & 0.683  &0.706 & 0.749 &  0.893\\
        &   \idnt w/ \quamsys{TCT}   &0.717 & 0.618 & 0.572 & 0.713 &0.653 & 0.701  & 0.706 & 0.752 & 0.901 \\
        &   \idnt w/ \cerberussys{TCT}   &0.680 & \textbf{0.637} & \textbf{0.598} & 0. &0.649 & \textbf{0.706}  &  \\
        \cmidrule{2-11}
       % &  \idnt w/ \sys{TCT}   &0.  & 0. & 0. &  &  &\\
       %  & \idnt w/ \sys{TCT}+Laff  &0.  &0.  &0. &  &  & \\
       %   & \idnt w/ \quamsys{TCT}  & 0. &0.  & 0. &  &   &\\
           
    \end{tabular}
    }
    \label{tab:main}
\end{table*}

==> tables/msmarco-v2.tex <==



\begin{table}
    \centering
    \caption{Effectiveness comparison* of \cerberus{} with hybrid and adaptive retrieval methods on TREC DL21 and DL22 test sets. The letter in subscript or superscript shows significant improvements (using paired t-test, $p<0.05$, with Bonferroni correction) over the corresponding baseline. The best score for each pipeline is highlighted in bold. }
    \vspace{-1em}
    {\small
     \setlength{\tabcolsep}{2.5pt}
    \begin{tabular}{llrrrr}
        \toprule
        \multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{2}{c}{$c=50$}&\multicolumn{2}{c}{$c=100$} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Dataset &Pipeline  &   nDCG@c & Recall@c &   nDCG@c  & Recall@c \\
    \midrule
  \multirow{12}{*}{\textbf{DL21}} & \bf\textsc{Hybrid } & \\
 \cmidrule{2-6}
   &  RRF>>MonoT5 [R] & 0.576 & 0.401  & 0.558 & 0.520  \\
   &  CC>>MonoT5 [C] & 0.584 & 0.419  & 0.569 & 0.545  \\
   &  \cerberus{}   & ${}^{R}$\bf{0.604}&${}^{R}$\bf0.444  & ${}^{RC}$\bf0.609 & ${}^{RC}$\bf0.609\\

   
    \cmidrule{2-6}
      &   \bf\textsc{Adaptive} & \\

    \cmidrule{2-6}
 \cellcolor{white} & BM25>>MonoT5 [B]   & 0.436 &0.242  &0.433 &0.331  \\
     &     \idnt w/ \sys{BM25} [G]    & 0.457 & 0.290  &0.465 &0.414  \\
        &  \idnt w/ \quamsys{BM25} [Q]   &0.478  & 0.310  &\bf0.499& 0.454  \\

        &   \idnt w/ \cerberussys{BM25}  & ${}^{GQ}_{B}$\textbf{0.503}& ${}^{GQ}_{B}$\textbf{0.364}  & ${}^{}_{B}$0.481 & ${}^{G}_{B}$ \bf0.463 \\
           
    \cmidrule{3-6}  
     &     \idnt w/ \sys{TCT} [G]   & 0.502 & 0.331  &\bf0.520&0.489  \\
        &  \idnt w/ \quamsys{TCT} [Q]   &0.491  & 0.311  &0.518& 0.477  \\

        &   \idnt w/ \cerberussys{TCT}    & ${}^{GQ}_{B}$\textbf{0.532}& ${}^{GQ}_{B}$\textbf{0.406} & ${}^{}_{B}$0.512 & ${}^{}_{B}$ \bf0.502 \\
                    \midrule

     \multirow{12}{*}{\textbf{DL22}} & \bf\textsc{Hybrid } & \\
   &  RRF>>MonoT5 [R]& 0.452 & 0.260  & 0.430 & 0.341 \\
   &  CC>>MonoT5 [C]& 0.459 & 0.278 & 0.433 & 0.362\\
   &  \cerberus{}   & ${}^{RC}$\bf0.481&${}^{R}$\bf0.297  & ${}^{RC}$\bf0.459 & ${}^{RC}$\bf0.389  \\
      % &  w/  \cerberus{} (BM25+TCT+$score_{diff}$) & \textbf{0.714} & \textbf{0.658}&\textbf{0.647} & \textbf{0.701} & \textbf{0.662} & \textbf{0.733} & 0.677 & 0.727 & 0.883 \\
       \cmidrule{2-6}
      &   \bf\textsc{Adaptive} & \\

    \cmidrule{2-6}
          & BM25>>MonoT5 [B]  & 0.290 &0.115  &0.275 &0.164   \\
      % &  \bf\textsc{Alternating} & &  &  &  & \\
     &     \idnt w/ \sys{BM25} [G]  & 0.287 & 0.121 &0.290 &0.191  \\
       % &  \idnt w/ \sys{BM25}+Laff  &0.707 &0.607  &0.548  &0.716 &0.643 &0.665 &0.708 &0.753 &0.898 \\
        &  \idnt w/ \quamsys{BM25} [Q]   &\bf0.308  & 0.135  &\bf0.303  &\bf0.196  \\
              
        &   \idnt w/ \cerberussys{BM25}   & ${}^{}_{}$\bf0.292  & ${}^{}_{}$\bf{0.137}   & ${}^{}_{}$0.284  & 0.195 \\
         \cline{3-6}
     &     \idnt w/ \sys{TCT} [G]    & 0.329 & 0.157  &\bf0.348&0.256  \\
        &  \idnt w/ \quamsys{TCT} [Q]   &0.329  & 0.155  &0.334& 0.237  \\

        &   \idnt w/ \cerberussys{TCT}    & ${}^{GQ}_{B}$\textbf{0.364}& ${}^{GQ}_{B}$\textbf{0.206}  & ${}^{}_{B}$0.342 & ${}^{}_{B}$ \bf0.260 \\
         \midrule
           
    \end{tabular}
    }
    \begin{minipage}{\columnwidth}
    \footnotesize{*We omit nDCG@10 measure because of space constraints and our focus is more on retrieval. Additionally, prior works find that nDCG@10 value saturates quickly during re-ranking, while evaluation at lower depths are able to further distinguish systems~\cite{plaid_repro}.}
\end{minipage}
    \vspace{-2em}
    \label{tab:msmarco-v2}
\end{table}

==> time_vs_calls_vs_perf.tex <==
\newcommand{\gt}[1]{\tiny{(\tikz\draw[green!60!black, fill=green!60!black] (0,0) -- (0.10,0) -- (0.05,0.10) -- cycle;{#1\%}})}

\newcommand{\rt}[1]{\tiny{(
    \tikz\draw[red, fill=red] (0,0) -- (0.10,0) -- (0.05,-0.10) -- cycle;%
    {#1\%})}}

\begin{table} %[b]
\centering
\caption{}
\label{tab:latency}
\begin{tabular}{rrclcl}
\toprule
& &\multicolumn{2}{c}{time (ms)}& \multicolumn{2}{c}{Recall@c}  \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} 
c & $|S|$  & \sys{BM25} & \quamsys{BM25} &\sys{BM25}  & \quamsys{BM25} \\
\midrule
50    & 10  & 2.64   &3.38\rt{28}  & 0.426 & 0.480\gt{12.7} \\
100   &  30 &  5.54     & 7.51\rt{35.6}  & 0.547 &0.611\gt{11.7}  \\
250   & 50  & 19.55    & 16.78\gt{14.2}  & 0.693 & 0.742\gt{7.1} \\
500    & 100  & 44.45   & 36.06\gt{18.9}  & 0.772 & 0.821\gt{6.3}\\
750  &  150 &  69.77   &57.36\gt{17.8}  & 0.811 & 0.849\gt{4.7}\\
1000  & 300  & 97.05   &95.72\gt{1.4}  & 0.833 &0.867\gt{4.1} \\
\bottomrule
\end{tabular}\vspace{-1em}
\end{table}
